Quantile-Optimal Policy Learning under Unmeasured Confounding

We study quantile-optimal policy learning where the goal is to find a policy whose reward distribution has the largest $\alpha$-quantile for some $\alpha \in (0, 1)$. We focus on the offline setting whose generating process involves unobserved confounders. Such a problem suffers from three main challenges: (i) nonlinearity of the quantile objective as a functional of the reward distribution, (ii) unobserved confounding issue, and (iii) insufficient coverage of the offline dataset. To address these challenges, we propose a suite of causal-assisted policy learning methods that provably enjoy strong theoretical guarantees under mild conditions. In particular, to address (i) and (ii), using causal inference tools such as instrumental variables and negative controls, we propose to estimate the quantile objectives by solving nonlinear functional integral equations. Then we adopt a minimax estimation approach with nonparametric models to solve these integral equations, and propose to construct conservative policy estimates that address (iii). The final policy is the one that maximizes these pessimistic estimates. In addition, we propose a novel regularized policy learning method that is more amenable to computation. Finally, we prove that the policies learned by these methods are $\tilde{\mathscr{O}}(n^{-1/2})$ quantile-optimal under a mild coverage assumption on the offline dataset. Here, $\tilde{\mathscr{O}}(\cdot)$ omits poly-logarithmic factors. To the best of our knowledge, we propose the first sample-efficient policy learning algorithms for estimating the quantile-optimal policy when there exist unmeasured confounding.

==> app_experiment.tex <==
\section{Experiment Details} \label{sec: app experiment}


\subsection{Algorithm Implementation Approximation}
\label{appendix:algo_approx}

The pessimistic policy learning algorithm implemented in our simulations is an approximation of the regularized pessimistic policy $\hat{\pi}_R$ defined in Algorithm 2 of the main paper, which is:
\[
\hat{\pi}_R = \arg\sup_{\pi} \inf_{h\in\mathcal{H}} \{ v(h,\pi) + \lambda_n \cdot \mathcal{E}_n(h) \}
\]
where $\mathcal{E}_n(h) = \mathcal{L}_n(h) - \inf_{h' \in \mathcal{H}} \mathcal{L}_n(h')$.

The implemented `PessimisticSolver` deviates from this formulation in the following manner:

\begin{enumerate}
    \item \textbf{Inner Maximization over $\theta$ (Test Functions)}: The term $\mathcal{L}_n(h)$ involves an inner maximization:
    \[
    \mathcal{L}_n(h) = \sup_{\theta\in\Theta} \left\{ \mathbb{E}_n[W(D;h) \cdot \theta(X,Z)] - \frac{1}{2n} \sum_{i=1}^n \theta^2(X_i,Z_i) \right\}
    \]
    In our implementation, we assume $\theta(X,Z) = \Psi(X,Z)^T \beta_\theta$, where $\Psi(X,Z)$ is the feature matrix for the test functions (denoted `self.Phi` in the code, a $d \times n$ matrix where $d$ is the number of basis functions for $\theta$, and $n$ is the number of samples). The objective for a fixed $h$ (and thus fixed $W(D;h)$ vector, denoted $W$) is to maximize $\frac{1}{n} W^T \Psi^T \beta_\theta - \frac{1}{2n} \beta_\theta^T \beta_\theta$ with respect to $\beta_\theta$.
    The code calculates the optimal $\beta_\theta^*$ (denoted `theta_star` in the code) using a ridge-like solution:
    \[
    \beta_\theta^* = (\Psi \Psi^T + \lambda_{ridge} I)^{-1} \Psi W
    \]
    This is the closed-form solution for $\beta_\theta$ if the objective for $\theta$ was $\frac{1}{n}W^T \Psi^T \beta_\theta - \frac{1}{2n} \beta_\theta^T (\Psi\Psi^T + \lambda_{ridge}I) \beta_\theta$ (assuming $\Psi\Psi^T$ is invertible, or more generally, using a regularized empirical norm for $\theta$). The term computed in the code for $\mathcal{L}_n(h)$ is then $\frac{1}{n} (W^T \Psi^T \beta_\theta^*) - \frac{1}{2n} (\beta_\theta^{*T} \beta_\theta^*)$. This provides an empirical estimate for the value of the inner supremum in $\mathcal{L}_n(h)$.

    \item \textbf{Outer Pessimistic Search}:
    \begin{itemize}
        \item First, a greedy estimate $\hat{\beta}_{greedy}$ is obtained by minimizing $\mathcal{L}_n(h(\cdot;\beta))$ with respect to $\beta$. This $\hat{\beta}_{greedy}$ corresponds to the $h$ that approximately gives $\inf_{h' \in \mathcal{H}} \mathcal{L}_n(h')$.
        \item Instead of directly solving the sup-inf problem for $\hat{\pi}_R$, the algorithm then samples $N_{pessim}$ candidate parameter vectors $\beta_s$ from a Gaussian distribution $N(\hat{\beta}_{greedy}, \Sigma)$. The covariance $\Sigma$ is either based on the inverse Hessian of $\mathcal{L}_n(\beta)$ at $\hat{\beta}_{greedy}$ or an isotropic covariance, scaled by $R_{scale} \propto 1/\sqrt{n_{train}}$. This sampling explores a neighborhood around $\hat{\beta}_{greedy}$.
        \item For each sampled $\beta_s$, the algorithm evaluates $v(h_s, \pi_s) = \mathbb{E}_{\pi_s} [h(A,X;\beta_s)]$, where $\pi_s$ is the greedy policy derived from $\beta_s$.
        \item The final pessimistic parameter $\hat{\beta}_{pessim}$ is the $\beta_s$ from the samples that \textit{minimizes} $v(h_s, \pi_s)$. The policy $\hat{\pi}_{pessim}$ is then derived from $\hat{\beta}_{pessim}$.
    \end{itemize}
\end{enumerate}

This procedure is a practical heuristic for achieving pessimism. The sampling around $\hat{\beta}_{greedy}$ acknowledges uncertainty in this initial estimate. The radius of sampling, controlled by $R_{scale}$, acts implicitly as a regularizer. Choosing $\beta_s$ that minimizes $v(h_s, \pi_s)$ from the samples is a form of worst-case selection within that neighborhood of uncertainty, aiming for a policy that is robust. While not a direct implementation of the augmented Lagrangian formulation of Algorithm 2, it shares the goal of mitigating over-optimism from purely greedy optimization, especially when $\mathcal{L}_n(h)$ might be flat or multimodal, or when $v(h,\pi)$ is sensitive to small changes in $h$. The scaling $R_{scale} \propto 1/\sqrt{n_{train}}$ acknowledges that with more data, the uncertainty (and thus the need for a large pessimistic neighborhood) should decrease, which is consistent with theoretical insights where error terms and confidence regions shrink with $n^{-1/2}$.

This approach was chosen for its computational tractability compared to a full saddle-point optimization, while still incorporating a notion of pessimistic evaluation.



In this section, we detail the data-generating process and the implementation of the algorithm used in the simulation experiment discussed in \S\ref{sec: experiment}.



\paragraph{Data Generating Process}
\begin{itemize}
    \item We set the context $X \sim N(0, 1)$ to be a one-dimensional Normal random variable.
    \item We set the instumental variable $Z \sim N(0, 1)$ to be a one-dimensional Normal random variable.
    \item We set the quantile of interest to be $\alpha = 0.2.$
    \item We set the error term induced by the unmeasured confounders $U$ to be $\epsilon \sim N(-\Phi^{-1}(\alpha), 1),$ where $\Phi(\cdot)$ is the CDF of a standard Normal distribution.
    \item To generate the binary action $A,$ we first set $t$ to be a variable such that with $p\%$ of the $n$ samples, it is a random noise: $t \sim N(0, 1).$ With the other samples, we let $t = X + Z + \epsilon + \gamma \mathbb{1}_{\{X > 0\}},$ where we will specify the value of $\gamma$ later.
    \item We generate $A \sim \text{Bernoulli}(q),$ where $q = \frac{\text{exp}(t)}{1 + \exp(t)}.$  
    \item We set the reward to be $Y = X + 3XA + \epsilon.$ 
\end{itemize}
It is easy to see that the oracle policy $\piestar$ is given by $\piestar(A=1 \given X) = \mathbb{1}_{\{X > 0\}}.$ Hence the value of $\gamma$ determines the level of concentration of the ODCP around the oracle policy. We set $\gamma = 8,$ so that around $(1-p)\%$ of the samples are concentrated around the optimal policy. We choose $p \in \{20, 50, 70\}$ in the experiments.

\paragraph{Algorithm Implementation}
Recall that given the offline dataset, we learn the policy by solving the following optimization problem:

\begin{align}
\piepessi_{R} &= \arg\sup_{\pie}\inf_{h\in \vH} \cbr{v(h, \pie) + \lambda_n\sup_{\theta\in\Theta}\cbr{\EE_n\sbr{W(D; h) \theta(\vX, \vZ)}-\frac 1 2 \nbr{\theta}_{n, 2}^2}}.
\end{align}

Since the solution does not admit a closed form, we perform gradient descent when optimizing over $h\in \vH.$ As $W(D; h)$ is not differentiable, we first smooth it by replacing the indicator function $\mathbb{1}\{Y \leq h(A, X)\}$ with $1 + \text{ exp}(-5[h(A, X) - Y]).$ We denote $W$ the vector in $\mathbb{R}^n$ such that $W_i = 1 + \text{exp}(-5[h(A_i, X_i) - Y_i]) - \alpha$ for a fixed $h.$ We choose $\vH$ and $\vTheta$ to be the linear function classes so that condition \ref{con: high probability event} holds by the results shown in \S\ref{app: bracketing concentration}. In particular, since $\hstaralpha(A, X) = X + AX$ by our choice, we can choose the feature map of $\cH=\{\cX\times \cA\rightarrow \beta_1^\top\phi(\cdot)\}$ to be $\phi(x, a) = (x, xa).$ Hence the realizability assumption in  Assumption \ref{asp: identifiability and realizability} holds. We also choose the feature map of the test function class $\vTheta$ to contain more polynomial features to ensure that the compatibility assumption \ref{asp: compatibility of test function class} holds. For $\Theta=\{\cX\times \cZ\rightarrow \beta_2^\top \psi(\cdot)\},$ we let $\psi(x, z) = (x, z, xz, x^2, z^2, xz^2, zx^2, x^3, z^3, x^2z^2).$ We denote $\Psi(X, Z)$ the $d$ by $n$ matrix such that its $i$-th column is $\psi(X_i, Z_i).$ As the condition of Theorem \ref{thm: convergence of sub-optimality reg} requires that $\lambda_n$ to be roughly $\tilde{\cO}(\eta_n^{-1})$ and that \S\ref{app: bracketing concentration} shows that $\eta_n = \tilde{\cO}(n^{-1/2}),$ we set $\lambda_n = 1.6n^{1/2}.$  After a random initialization of $\pi$ and $h \in \vH,$ we repeatedly carry out the following procedures to update $\pi:$

\begin{itemize}
    \item By setting the gradient to $0,$ we derive that $\theta^{*} := {\beta^{*}}^T \phi(\cdot) \in \Theta$ solves
    \begin{align*}
        \sup_{\theta\in\Theta}\cbr{\EE_n\sbr{W(D; h) \theta(\vX, \vZ)}-\frac 1 2 \nbr{\theta}_{n, 2}^2},
    \end{align*}
    where $\beta^{*} := \psi(X, Z)(\psi(X, Z)^T\psi(X, Z))^{-1}W.$    
    \item We perform gradient descent on $h \in \vH$ to minimize $v(h, \pie) + \lambda_n \cbr{\EE_n\sbr{W(D; h) \theta^{*}(\vX, \vZ)}-\frac 1 2 \nbr{\theta^{*}}_{n, 2}^2}.$ Let $h^{*}$ be the argmin.
    \item We then update $\pi$ by solving the linear programming problem that maximizes $v(h^{*}, \pie)$ with respect to $\pi,$ subject to the constraint that each of $\pi(X_i, Z_i)$ is a probability distribution over $A.$
\end{itemize}

==> related_work.tex <==
% !TEX root = paper.tex


==> temproof.tex <==
{\red Original proof}
Let $\theta_k^*=\arg\sup_{\theta_k\in\Theta_k} \EE_{\mu_k}\sbr{\alpha^\pi_k(\vh_k, \cY_k) \theta_k(\cZ_k)} - \frac 1 2 \nbr{\theta_k}_{\mu_k, 2}^2$. Suppose that $\EE_{\mu_k}\sbr{\alpha^\pi_k(\vh_k, \cY_k) \theta_k^*(\cZ_k)}=\beta \nbr{\theta_k^*}_{\mu_k, 2}^2$. By definition of $\theta_k^*$, we have that
\begin{align}\label{eq:beta-LB}
    \rbr{\beta-\frac 1 2} \nbr{\theta_k^*}_{\mu_k, 2}^2=\sup_{\theta_k\in\Theta_k} \EE_{\mu_k}\sbr{\alpha^\pi_k(\vh_k, \cY_k) \theta_k(\cZ_k)} - \frac 1 2 \nbr{\theta_k}_{\mu_k, 2}^2\ge 0,
\end{align}
where the last inequality holds by plugging in $\theta_k=0$.
We plug in $\kappa \theta_k^*$ in \eqref{eq:L_D(h_CI)-LB-1} where $0<\kappa\le 2/3$. Note that $\Theta_k$ is star shaped. Thus, we have $\kappa \theta_k^*\in\Theta_k$ and it holds on event $\cE_{k, 3}$ that
\begin{align}\label{eq:L_D(h_CI)-LB-2}
    \cL_{k,\cD_k}^\pi(\vh_k) 
    &\gtrsim \kappa\rbr{\beta-\frac 3 4 \kappa}\nbr{\theta_k^*}_{\mu_k, 2}^2 - \eta_{\Theta_k, \vH_k, \cD_k}L_\alpha \kappa\nbr{\theta_k^*}_{\mu_k, 2} - \rbr{\eta_{\Theta_k, \vH_k, \cD_k}^2 + \frac 1 4\eta_{\Theta_k, \cD_k}^2}.
\end{align}
Recall that it holds on event $\cE_2$ that
\begin{align}\label{eq:19}
    \nbr{\vcL_{\cD}^\pi(\vh)}_\infty
    &\le \nbr{\vcL_{\cD}^\pi(\hat\vh^\pi)}_\infty + e_\cD\nend
    &\le \nbr{\vcL_{\cD}^\pi(\vh^{\pi, *})}_\infty + e_\cD\nend
    &\lesssim 4\varepsilon_{\vH} + \rbr{2 L_\alpha^2+L_\alpha+\frac 1 4}\max_{k\in\{1, \cdots, K\}}\eta_{\Theta_k, \cD_k}^2 + e_\cD,
\end{align}
where the last inequality holds by \eqref{eq:L_D(h^*)-UB-2}. Combining \eqref{eq:L_D(h_CI)-LB-2} with \eqref{eq:19} and letting $\cE_{k, 4}=\cE_2\cap\cE_{k, 3}$, it holds on event $\cE_{k, 4}$ that
\begin{align}\label{eq:quadratic inequation}
    \kappa\rbr{\beta-\frac 3 4 \kappa}\nbr{\theta_k^*}_{\mu_k, 2}^2 - \eta_{\Theta_k, \vH_k, \cD_k}L_\alpha \kappa\nbr{\theta_k^*}_{\mu_k, 2} - \Delta_{k, \cD} \lesssim 0,
\end{align}
where $\Delta_{\cD, k}=\eta_{\Theta_k, \vH_k, \cD_k}^2 + \frac 1 4\eta_{\Theta_k, \cD_k}^2+4\varepsilon_{\vH} + \rbr{2 L_\alpha^2+L_\alpha+\frac 1 4}\cdot \max_{k\in\{1, \cdots, K\}}\eta_{\Theta_k, \cD_k}^2 + e_\cD$ and $\cP(\cE_{k, 4})\ge 1-2(K+1)\xi$. 
We consider the following two cases
\paragraph{Case (i).} $\nbr{\theta_k^*}_{\mu_k, 2}>0$ holds on event $\cE_{k, 5}$. 

on event $\cE_{k, 4}\cap \cE_{k, 5}$, we restrict $\kappa$ by $0<\kappa < 2/3$.
We then have $\beta-3\kappa/4> \beta-1/2\ge 0$ where the last inequality holds by \eqref{eq:beta-LB} and noting that $\nbr{\theta_k^*}_{\mu_k, 2}>0$.
Therefore, solving the quadratic inequation \eqref{eq:quadratic inequation}, for any $0<\kappa <2/3$, it holds on event $\cE_{k, 4}\cap \cE_{k, 5}$ that
\begin{align}
    0< \nbr{\theta_k^*}_{\mu_k, 2}\lesssim \frac{\sqrt{\rbr{\eta_{\Theta_k, \vH_k, \cD_k}L_\alpha \kappa}^2+\kappa\rbr{4\beta-3\kappa}\Delta_{k, \cD}}+\eta_{\Theta_k, \vH_k, \cD_k}L_\alpha \kappa}{\kappa\rbr{2\beta-\frac 3 2 \kappa}}.
\end{align}
Plug in $\kappa=1/3$, it holds on event $\cE_{k, 4}\cap \cE_{k, 5}$ that $\nbr{\theta_k^*}_{\mu_k, 2}>0$ and that
\begin{align}
    \nbr{\theta_k^*}_{\mu_k, 2}^2
    &\lesssim 4\rbr{\sqrt{\rbr{\eta_{\Theta_k, \vH_k, \cD_k}L_\alpha}^2+3\Delta_{k, \cD}}+\eta_{\Theta_k, \vH_k, \cD_k}L_\alpha}^2\nend
    &\le 8\rbr{2\rbr{\eta_{\Theta_k, \vH_k, \cD_k}L_\alpha}^2+3\Delta_{k, \cD}}\nend
    &\le 24\rbr{ \rbr{\frac 2 3 L_\alpha^2 + 1}\eta_{\Theta_k, \vH_k, \cD_k}^2 + \rbr{2 L_\alpha^2+L_\alpha+\frac 1 2} \max_{k\in\{1, \cdots, K\}}\eta_{\Theta_k, \cD_k}^2 + 4\varepsilon_\vH + e_\cD}\nend
    &\le 24\tilde \Delta_{k,\cD},
\end{align}
where $\tilde \Delta_{k, \cD}=\rbr{\frac 2 3 L_\alpha^2 + 1}\eta_{\Theta_k, \vH_k, \cD_k}^2 + \rbr{2 L_\alpha^2+L_\alpha+\frac 1 2} \max_{k\in\{1, \cdots, K\}}\eta_{\Theta_k, \cD_k}^2 + 4\varepsilon_\vH + e_\cD$.
Recall the definition of $\theta_k^*$ by $\theta_k^*=\arg\sup_{\theta_k\in\Theta_k} \EE_{\mu_k}\sbr{\alpha^\pi_k(\vh_k, \cY_k) \theta_k(\cZ_k)} - \frac 1 2 \nbr{\theta_k}_{\mu_k, 2}^2$ and the definition of $\cL^\pi_k(\vh_k)$ in \eqref{eq:population loss-def}, it holds on event $\cE_{k, 4}\cap \cE_{k, 5}$ that
\begin{align}
    \cL^\pi_k(\vh_k) 
    &=\EE_{\mu_k}\sbr{\alpha^\pi_k(\vh_k, \cY_k) \theta_k^*(\cZ_k)} - \frac 1 2 \nbr{\theta_k^*}_{\mu_k, 2}^2\nend
    & = (\beta-\frac 1 2)\nbr{\theta_k^*}_{\mu_k, 2}^2\nend
    &\lesssim \eta_{\Theta_k, \vH_k, \cD_k} L_\alpha \nbr{\theta_k^*}_{\mu_k, 2} + \frac 3 2 \Delta_{k, \cD}\nend
    &<9 \tilde\Delta_{k, \cD},
\end{align}
where the first inequality holds by replacing \eqref{eq:quadratic inequation} and plugging in $\kappa=2/3$ The last inequality holds by noting that $\tilde\Delta_{k, \cD}>\Delta_{k, \cD}$ and that $\sqrt{24}\eta_{\Theta_k, \vH_k, \cD_k} L_\alpha \le 15\tilde\Delta_{k, \cD}/2$.


\paragraph{Case (ii).} $\nbr{\theta_k^*}_{\mu_k, 2}=0$ on event $\bar\cE_{k, 5}$, thereby 
\begin{align}
    \cL_k^\pi(\vh_k)=\EE_{\mu_k}\sbr{\alpha^\pi_k(\vh_k, \cY_k) \theta_k^*(\cZ_k)} - \frac 1 2 \nbr{\theta_k^*}_{\mu_k, 2}^2=0.
\end{align}

Combining case (i) and case (ii), we see that on event $\cE_{k, 4}$ it holds that
\begin{align}
    \cL^\pi_k(\vh_k) \lesssim 9\tilde \Delta_{k, \cD}.
\end{align}
Define $\cE_6=\cap_{k=1}^K \cE_{k, 4}$. Recall that $\cE_{k, 4}=\cE_2\cap\cE_{k, 3}$, Thereby, we have that $\cE_6 = \cE_2 \cap (\cap_{k=1}^K \cE_{k, 3})$ and that $\cP(\cE_6)\ge 1- 4K\xi$. Moreover, on event $\cE_6$, it holds that
\begin{align}
    \nbr{\vcL^\pi_{\cD}(\vh^{\pi, *})}_\infty - \nbr{\vcL^\pi_{ \cD}(\hat\vh^\pi)}_\infty\lesssim 4\varepsilon_{\vH} + \rbr{2 L_\alpha^2+L_\alpha+\frac 1 4}\max_{k\in\cbr{1, \cdots, K}}\eta_{\Theta_k, \cD_k}^2, 
\end{align}
and that
\begin{align}
    \cL^\pi_k(\vh_k) \lesssim 9\tilde \Delta_{k, \cD}, 
\end{align}
where $\tilde \Delta_{k, \cD}=\rbr{\frac 2 3 L_\alpha^2 + 1}\eta_{\Theta_k, \vH_k, \cD_k}^2 + \rbr{2 L_\alpha^2+L_\alpha+\frac 1 2} \max_{k\in\{1, \cdots, K\}}\eta_{\Theta_k, \cD_k}^2 + 4\varepsilon_\vH + e_\cD$.
Therefore, we complete the proof of Theorem \ref{thm:Fast rate}.
